DistillPose: Lightweight Camera Localization Using Auxiliary Learning

We propose a lightweight retrieval-based pipeline to predict 6DOF camera poses from RGB images. Our pipeline uses a convolutional neural network (CNN) to encode a query image as a feature vector. A nearest neighbor lookup finds the pose-wise nearest database image. A siamese convolutional neural network regresses the relative pose from the nearest neighboring database image to the query image. The relative pose is then applied to the nearest neighboring absolute pose to obtain the query image's final absolute pose prediction. Our model is a distilled version of NN-Net that reduces its parameters by 98.87%, information retrieval feature vector size by 87.5%, and inference time by 89.18% without a significant decrease in localization accuracy.

==> sections/related-work.tex <==
% !TeX root = ../root.tex

\input{figures/layerwise-model.tex}

% \section{Related Work}

% \textbf{3D Model-Based Localization.}
% Given a 3D model for a scene and a query image, feature descriptors \cite{lowe2004Sift,bay2008Surf,calonder2010BRIEFDescriptor,rublee2011ORB,yi2016LIFT} from the query image could be used to query a feature descriptor database.
% This establishes a set of 2D to 3D point correspondences based on which pose estimation algorithm using PnP \cite{szeliski2010computerVisionBook} and RANSAC \cite{fischler1981randomRansac} can then be used to obtain a camera pose estimate.
% \cite{sattler2012improvingActiveSearch} introduces an efficient search method to match image features and 3D scene points.
% Unlike traditional pipelines where image features are used to query a point cloud database (with corresponding features), \cite{sattler2012improvingActiveSearch} actively searches for additional matches based on 2D-to-3D and 3D-to-2D search.
% 3D-to-2D search is more efficient due to the smaller search space.
% This mechanism achieves stellar results on indoor datasets like the Seven Scenes \cite{glocker2013SevenScenes}.

% \textbf{Scene Coordinate Regression.}
% A regressor is trained for each scene to predict the 3D scene coordinates of the corresponding image pixels.
% Usually, either convolutional neural networks (CNNs) or random forests are used.
% \cite{shotton2013SCoReForest} uses random forests \cite{criminisi2013decisionForestsBook} to predict 3D coordinates using RGB images, depth images or both; It does not use the entire image to predict the 3D points but rather takes single pixels as input.
% This leads to fairly smaller model sizes.
% The forest regressors are used in a RANSAC loop \cite{fischler1981randomRansac} where a pose is refined iteratively.
% On each iteration, a set of 2D pixels is sampled, the regressor is used to predict their 3D scene coordinates, and the pose is refined.
% The pose with the highest inlier count is then used as the final prediction.
% \cite{brachmann2017Dsac} develops a differentiable RANSAC \cite{fischler1981randomRansac} pipeline for pose estimation.
% It incorporates the pose hypotheses selection and refinement in an end-to-end trainable pipeline which, in turn, improves the results of \cite{shotton2013SCoReForest}.

% \textbf{Absolute Pose Regression.}
% Methods in this bucket learn to regress a 7-dimensional vector representing the absolute pose from RGB images.
% \cite{kendall2015posenet} introduced the first absolute pose regression model on top of CNNs.
% They use a GoogLeNet \cite{szegedy2015goingGoogLeNet} backbone to transform scene images to feature vectors;
% A fully-connected layer regresses both absolute translations and rotation unit quaternions.
% \cite{kendall2016modellingBayesianPoseNet} aims at modelling uncertainty in the pose estimation task by using Bayesian Neural Networks \cite{gal2015bayesianNeuralNets}.
% \cite{kendall2017geometricLossFunctions} reformulates the pose regression task introduced in \cite{kendall2015posenet} to make use of geometric re-projections and homoscedastic uncertainty \cite{kendall2017uncertaintiesHomoscedastic}.
% \cite{walch2017LSTMPose} introduced a new LSTM-based correlation layer on top of PoseNet \cite{kendall2015posenet} feature vectors;
% \cite{walch2017LSTMPose} applies LSTM units both horizontally (right-to-left and left-to-right) and vertically (bottom-up and top-down).
% While this LSTM-based correlation step slightly improves the results on indoor pose localization (in comparison with \cite{kendall2015posenet}), it drastically improves the localization performance on outdoor datasets.
% \cite{valada2018vlocnet} reformulates the camera localization problem as a tracking problem.
% Their model learns to predict current frame's absolute pose given current frame's RGB image and previous frame's absolute pose.
% \cite{melekhov2017imageHourGlassPose} introduces an encoder-decoder architecture (i.e. \textit{hourglass architecture} \cite{newell2016stackedHourglassNetworks});
% This architecture seems to consistently improve the translational error; However, it does not show a consistent improvement on the rotational error.
% MapNet \cite{brahmbhatt2018MapNet} enforces odometric pose constraints by employing absolute and relative pose regression losses in their training pipeline.
% These constraints improve the performance of the absolute pose regression significantly.
% VidLoc \cite{clark2017vidloc} proposes to use a bi-directional recurrent neural network to embed temporal contextual information in the final pose regressor.

% \textbf{Information Retrieval.}
% Methods in this bucket decompose the camera localization problem into two sub-problems: information retrieval and relative pose regression.
% Information retrieval finds the nearest neighbor for a given query image.
% Relative pose regression estimates the change in pose from the nearest neighbor to the query image.

% NN-Net \cite{laskar2017camera} uses two siamese branches of ResNet34 to predict a feature vector per image and regresses relative translation and rotation.
% For each query image, $N$ nearest training neighbors are fetched.
% A filtering post-processing step triangulates the final absolute pose.
% RelocNet \cite{balntas2018relocnet} correlates learned features to changes in the viewing camera frustum to improve nearest neighbor retrieval.
% Unlike \cite{laskar2017camera}, \cite{balntas2018relocnet} regresses a transformation matrix (rather than translations and unit quaternions).
% CamNet \cite{ding2019camnet} achieves state-of-the-art performance due to two main ideas: a) they break the relative pose estimation problem into two sub-problems (fine and precise modules); b) they use rgb-based (i.e. angle loss, triplets loss) and depth-based (i.e. frustum loss) pose constraints.
% Auxiliary learning allows CamNet to learn and use depth-based features in their nearest neighbor retrieval component.
% EssNet \cite{zhou2020learnEssNet} shows that relative pose regression overfits on a given dataset rather than generalize to totally unseen scenes.
% \cite{zhou2020learnEssNet} shows that using a feature descriptor (i.e. SIFT \cite{lowe2004Sift}) and 5-Point solver \cite{nister2004efficient5PTSolver} outperform all learning-based methods and generalizes better.
% In their learning-based model, unlike \cite{kendall2015posenet,laskar2017camera,ding2019camnet}, their model uses essential matrices to represent poses.
% ExReNet \cite{winkelbauer2020learningExReNet} addresses the overfitting problems (presented in \cite{zhou2020learnEssNet}) by training using synthetic scenes and employing correlation layers.
% They also regress a scale signal to improve the results of RANSAC filtering proposed in \cite{laskar2017camera}.

% In this work, we remove the need for a RANSAC pose filtering altogether by using a single nearest neighbor in our inference pipeline.
% Unlike previous works, our goal is to distill a large model (i.e. NN-Net \cite{laskar2017camera}) into a smaller form factor using auxiliary learning and layerwise training.

==> tables/pose-regression.tex <==
\begin{table*}
    \centering
    \caption{
      \textbf{Impact of Homoscedastic Loss Term Weighting on Relative Pose Prediction.}
      ``PL'' refers to the L1 pose loss (Sec. \ref{section:model-b}).
      ``EA'' refers to enforcing the angular distance directly on the embedding space (Sec. \ref{section:enforcing-angular-distance}).
      ``EF'' refers to enforcing the bilateral frustum distance directly on the embedding space (Sec. \ref{section:enforcing-frustum-distance}).
      ``PA'' refers to predicting the angular distance (Sec. \ref{section:predicting-angular-distance}).
      ``PF'' refers to predicting the bilateral frustum distances (Sec. \ref{section:predicting-frustum-distances}).
      ``H'' refer to model variants where a homoscedastic loss has been used to learn an optimal weighting for loss terms.
      Highlighting here refers to best value within the vertical lines (i.e. comparing variants with and without a homoscedastic).
    }
    \label{table:impact-of-homoscedastic-prediction}
    \centerline{
      \footnotesize
        \begin{tabular}{c|ccccccc|c}
            \toprule
            Scene &                           Chess &                          Office &                           Stairs &                            Heads &                             Fire &                         Pumpkin &                      Redkitchen &                          Average \\
            \midrule
            NN-Net \cite{laskar2017camera} &                    0.13m, 6.46\degree &                    0.21m, 7.35\degree &                    0.27m, 11.82\degree &                    0.14m, 12.34\degree &                    0.26m, 12.72\degree &                    0.24m, 6.35\degree &                    0.24m, 8.03\degree &                     0.21m, 9.30\degree \\
            \midrule
            L1/P1 (PL+EA)                     &  \textbf{0.16}m, \textbf{7.51}\degree &  \textbf{0.25}m, \textbf{8.40}\degree &  \textbf{0.34}m, \textbf{13.68}\degree &                    0.21m, 13.35\degree &  \textbf{0.27}m, \textbf{14.64}\degree &  \textbf{0.21}m, \textbf{8.16}\degree &  \textbf{0.28}m, \textbf{8.10}\degree &  \textbf{0.24}m, \textbf{10.55}\degree \\
            L1/P1 (PL+EA+H)                   &                    0.19m, 7.81\degree &                    0.27m, 8.94\degree &                    0.36m, 14.51\degree &  \textbf{0.20}m, \textbf{11.23}\degree &                    0.31m, 17.69\degree &                    0.23m, 8.41\degree &           \textbf{0.28}m, 8.60\degree &                    0.26m, 11.03\degree \\
            \midrule
            L1/P1 (PL+EF)                     &                    0.16m, 7.66\degree &  \textbf{0.23}m, \textbf{8.99}\degree &           \textbf{0.39}m, 13.70\degree &                    0.26m, 14.17\degree &                    0.28m, 13.73\degree &  \textbf{0.19}m, \textbf{7.08}\degree &           0.26m, \textbf{8.82}\degree &                    0.25m, 10.59\degree \\
            L1/P1 (PL+EF+H)                   &  \textbf{0.15}m, \textbf{7.41}\degree &           \textbf{0.23}m, 9.06\degree &  \textbf{0.39}m, \textbf{12.86}\degree &  \textbf{0.19}m, \textbf{11.83}\degree &  \textbf{0.26}m, \textbf{13.50}\degree &                    0.20m, 8.04\degree &           \textbf{0.25}m, 9.00\degree &  \textbf{0.24}m, \textbf{10.24}\degree \\
            \midrule
            L1/P1 (PL+PA)                     &                    0.17m, 7.14\degree &           0.25m, \textbf{8.72}\degree &                    0.34m, 15.38\degree &                    0.20m, 12.07\degree &  \textbf{0.27}m, \textbf{13.22}\degree &                    0.22m, 8.04\degree &                    0.27m, 9.10\degree &                    0.25m, 10.52\degree \\
            L1/P1 (PL+PA+H)                   &  \textbf{0.15}m, \textbf{6.86}\degree &           \textbf{0.24}m, 8.74\degree &  \textbf{0.31}m, \textbf{12.19}\degree &  \textbf{0.17}m, \textbf{11.15}\degree &           \textbf{0.27}m, 13.68\degree &  \textbf{0.19}m, \textbf{7.53}\degree &  \textbf{0.25}m, \textbf{8.83}\degree &   \textbf{0.23}m, \textbf{9.85}\degree \\
            \midrule
            L1/P1 (PL+PF)                     &           \textbf{0.16}m, 7.86\degree &                    0.25m, 8.65\degree &                    0.40m, 14.88\degree &                    0.19m, 14.15\degree &           \textbf{0.28}m, 12.91\degree &  \textbf{0.20}m, \textbf{7.65}\degree &                    0.27m, 9.11\degree &                    0.25m, 10.74\degree \\
            L1/P1 (PL+PF+H)                   &  \textbf{0.16}m, \textbf{7.03}\degree &  \textbf{0.23}m, \textbf{8.36}\degree &  \textbf{0.36}m, \textbf{14.34}\degree &  \textbf{0.14}m, \textbf{12.05}\degree &           0.29m, \textbf{12.81}\degree &                    0.21m, 8.58\degree &  \textbf{0.24}m, \textbf{8.62}\degree &  \textbf{0.23}m, \textbf{10.26}\degree \\
            \bottomrule
        \end{tabular}
    }
  \end{table*}
